Vision Transformer-based Model for Severity Quantification of Lung Pneumonia Using Chest X-ray Images

To develop generic and reliable approaches for diagnosing and assessing the severity of COVID-19 from chest X-rays (CXR), a large number of well-maintained COVID-19 datasets are needed. Existing severity quantification architectures require expensive training calculations to achieve the best results. For healthcare professionals to quickly and automatically identify COVID-19 patients and predict associated severity indicators, computer utilities are needed. In this work, we propose a Vision Transformer (ViT)-based neural network model that relies on a small number of trainable parameters to quantify the severity of COVID-19 and other lung diseases. We present a feasible approach to quantify the severity of CXR, called Vision Transformer Regressor Infection Prediction (ViTReg-IP), derived from a ViT and a regression head. We investigate the generalization potential of our model using a variety of additional test chest radiograph datasets from different open sources. In this context, we performed a comparative study with several competing deep learning analysis methods. The experimental results show that our model can provide peak performance in quantifying severity with high generalizability at a relatively low computational cost. The source codes used in our work are publicly available at https://github.com/bouthainas/ViTReg-IP.

==> Bouthaina Slika-Severity Prediction/utfsym/doc/symbole.tex <==
\section{Unicode-Symbol-Blöcke}
\label{sec:unicodesymbole}
\newcommand{\utab}[1]{\label{utab:#1}\includegraphics[scale=0.9]%
	{Abbildungen/table#1.pdf}}
\subsection{Miscellaneous Symbols and Arrows (2600-26FF)}
\utab{02600-026FF}

\subsection{Dingbats (2700-27BF)}
\utab{02700-027BF}

\subsection{Mahjong Tiles (1F000-1F02F)}
\utab{1F000-1F02F}

\subsection{Domino Tiles (1F030-1F09F)}
\utab{1F030-1F09F}

\subsection{Playing Cards (1F0A0-1F0FF)}
\utab{1F0A0-1F0FF}

\subsection{Miscellaneous Symbols and Pictographs (1F300-1F5FF)}
\utab{1F300-1F5FF}

\subsection{Emoticons / Emoji (1F600-1F64F)}
\utab{1F600-1F64F}

\subsection{Transport and Map Symbols (1F680-1F6FF)}
\utab{1F680-1F6FF}

==> utfsym/doc/symbole.tex <==
\section{Unicode-Symbol-Blöcke}
\label{sec:unicodesymbole}
\newcommand{\utab}[1]{\label{utab:#1}\includegraphics[scale=0.9]%
	{Abbildungen/table#1.pdf}}
\subsection{Miscellaneous Symbols and Arrows (2600-26FF)}
\utab{02600-026FF}

\subsection{Dingbats (2700-27BF)}
\utab{02700-027BF}

\subsection{Mahjong Tiles (1F000-1F02F)}
\utab{1F000-1F02F}

\subsection{Domino Tiles (1F030-1F09F)}
\utab{1F030-1F09F}

\subsection{Playing Cards (1F0A0-1F0FF)}
\utab{1F0A0-1F0FF}

\subsection{Miscellaneous Symbols and Pictographs (1F300-1F5FF)}
\utab{1F300-1F5FF}

\subsection{Emoticons / Emoji (1F600-1F64F)}
\utab{1F600-1F64F}

\subsection{Transport and Map Symbols (1F680-1F6FF)}
\utab{1F680-1F6FF}
